Enhancing the Learning Experience: Using Vision-Language Models to Generate Questions for Educational Videos

Web-based educational videos offer flexible learning opportunities and are becoming increasingly popular. However, improving user engagement and knowledge retention remains a challenge. Automatically generated questions can activate learners and support their knowledge acquisition. Further, they can help teachers and learners assess their understanding. While large language and vision-language models have been employed in various tasks, their application to question generation for educational videos remains underexplored. In this paper, we investigate the capabilities of current vision-language models for generating learning-oriented questions for educational video content. We assess (1) out-of-the-box models' performance; (2) fine-tuning effects on content-specific question generation; (3) the impact of different video modalities on question quality; and (4) in a qualitative study, question relevance, answerability, and difficulty levels of generated questions. Our findings delineate the capabilities of current vision-language models, highlighting the need for fine-tuning and addressing challenges in question diversity and relevance. We identify requirements for future multimodal datasets and outline promising research directions.

==> tables/ablation_metrics.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Comparing the fine-tuned \textit{PG-Video-LLaVA}~\cite{munasinghe2023PGVideoLLaVA} and \textit{Video-LLaMA}~\cite{damonlpsg2023videollama} regarding the \textit{BLEU}~\cite{bleu} (\textit{B}), \textit{ROUGE}~\cite{rouge} (\textit{R}) and \textit{BertScore}~\cite{bertscore} (\textit{BE}) metrics on different modalities (normal, visual only, audio only).}
\label{tab:ablation_metrics}
\begin{tabular}{llll}
  \toprule
  \textbf{Model} & \textbf{B~\cite{bleu}} & \textbf{R~\cite{rouge}} & \textbf{BE~\cite{bertscore}}\\
  \midrule
  PG-Video-LLaVA & 4.19 & 0.19 & 0.87\\
  PG-Video-LLaVA (visual) & 4.52 & 0.20 & 0.87\\
  PG-Video-LLaVA (audio) & 0.00 & 0.00 & 0.00\\
  Video-LLaMA & 3.48 & 0.15 & 0.86 \\
  Video-LLaMA (visual) & 1.18 & 0.07 & 0.42\\
  Video-LLaMA (audio) & 2.27 & 0.09 & 0.45\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/ablation_metrics_new.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Comparing fine-tuned \textit{PG-Video-LLaVA} %~\cite{munasinghe2023PGVideoLLaVA} 
and \textit{Video-LLaMA} %~\cite{damonlpsg2023videollama}
regarding \textit{BLEU} %~\cite{bleu}
(\textit{B}), \textit{ROUGE} %~\cite{rouge}
(\textit{R}) and \textit{BertScore} %~\cite{bertscore}
(\textit{BE}) on different modalities (multimodal, visual only, audio only).}
\label{tab:ablation_metrics}
\begin{tabular}{llll}
  \toprule
  \textbf{Model} & \textbf{B~\cite{bleu}} & \textbf{R~\cite{rouge}} & \textbf{BE~\cite{bertscore}}\\
  \midrule
  PG-Video-LLaVA & 0.00 & 0.42 & 0.22\\
  Video-LLaMA & 0.00 & 0.25 & 0.21 \\
  \midrule
  PG-Video-LLaVA (visual) & 0.00 & 0.37 & 0.34\\
  PG-Video-LLaVA (audio) & 0.00 & 0.00 & 0.00\\
  Video-LLaMA (visual) & 0.00 & 0.24 & 0.19\\
  Video-LLaMA (audio) & 0.00 & 0.25 & 0.17\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/blooms_taxonomy.tex <==
\begin{table*}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Possible levels of questions and their examples~\cite{ICWSM18LearningQ} regarding Bloom's taxonomy~\cite{blooms_taxonomy}.}
\label{tab:blooms_taxonomy}
\begin{tabular}{lll}
  \toprule
  \textbf{Level} & \textbf{Description} & \textbf{Example}\\
  \midrule
  Remembering & Retrieving relevant knowledge from long-term memory. & How big is an atom?\\
  \midrule
  Understanding & \makecell[l]{Questions that are solved by constructing\\ meanings from content.} & Why do some plankton migrate vertically?\\
  \midrule
  Applying & Answering using f.e. a specific procedure. & \makecell[l]{If I double the area and take half\\ of the fraction, do I get the same result?}\\
  \midrule
  Analyzing & \makecell[l]{Content must be broken down into individual parts\\ to understand the purpose.} & Why did sea levels drop during the ice age?\\
  \midrule
  Evaluating & Evaluating information based on criteria & \makecell[l]{Will all the cultures merge into one big culture,\\ due to the fading genetic distinctions?}\\
  \midrule
  Creating & Putting information together to design a new structure.  & \makecell[l]{Can somebody please explain to me what\\ marginal benefits are and give me some examples?}\\
  \bottomrule
\end{tabular}
\end{table*}

==> tables/data_finetuned_questionwords.tex <==
\begin{table*}[ht]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{The percentage distribution of different question words of \textit{PG-Video-LLaVA} (P-V-L) and \textit{Video-LLaMA} (V-LM) on the generated questions after fine-tuning and usage of different modalities (multimodal, visual only [V], audio only [A]). \textit{None} defines generated questions without a question word.
Additionally, the statistics of the ground-truth training questions are given (GT).}
\label{tab:finetune_questionwords}
\begin{tabular}{lrrrrrrrrrr}
  \toprule
  \textbf{Model} & \textbf{Where} & \textbf{Who} & \textbf{When} & \textbf{What} & \textbf{Why} & \textbf{Whose}
   & \textbf{Whom} & \textbf{Which} & \textbf{How} & \textbf{None}\\
  \midrule
  P-V-L & 0.00 & 0.01 & 0.01 & 69.06 & 2.19 & 0.00 & - & 0.00 & 13.46 & 15.26 \\
  P-V-L (V) & 0.00 & 0.01 & 0.00 & 46.89 & 9.57 & 0.00 & - & 0.00 & 34.12 & 9.42 \\
  P-V-L (A) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & - & 0.00 & 0.00  & 0.00\\
  
  V-LM & 0.07 & 0.13 & 0.52 & 34.34 & 1.94 & 0.00 & - & 0.44  & 28.08 & 34.47 \\
  V-LM (V) & 0.06 & 0.16 & 0.34 & 31.65 & 1.62 & 0.00 & - & 0.30 & 29.18 & 36.68 \\
  V-LM (A) & 0.05 & 0.09 & 0.45 & 32.98 & 2.25 & 0.00 & - & 0.58 & 29.91 & 33.69 \\
  \midrule
  GT & 0.96 & 0.38 & 2.06 & 14.51 & 9,76 & 0.00 & - & 0.58 & 13.67 & 58.07\\
  \bottomrule
\end{tabular}
\end{table*}

==> tables/data_statistics_finetuned.tex <==
\begin{table}[ht]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Statistics about the output of \textit{PG-Video-LLaVA} %}~\cite{munasinghe2023PGVideoLLaVA}
and \textit{Video-LLaMA} %~\cite{damonlpsg2023videollama} 
after fine-tuning.
Text length: \textit{min} stands for minimum, \textit{Avg.} for average, \textit{Max} for maximum. \textit{Flesch} is the value of the Flesch-Reading-Ease readability metric.}
\label{tab:finetune_stats}
\begin{tabular}{lrrrr}
  \toprule
  \textbf{Model} & \textbf{Min} & \textbf{Avg.} & \textbf{Max} & \textbf{Flesch}\\
  \midrule
  PG-Video-LLaVA & 1 & 15.80 & 857 & 72.84 \\
  PG-Video-LLaVA (visual) & 3 & 10.84 & 104 & 77.46 \\
  PG-Video-LLaVA (audio) & 0 & 0.00 & 0 & 0.00 \\
  Video-LLaMA & 4 & 57.70 & 272 & 51.08 \\
  Video-LLaMA (visual) & 2 & 25.79 & 283 & 58.24 \\
  Video-LLaMA (audio) & 5 & 36.42 & 230 & 88.78 \\
  \midrule
  GT & - & - & - & - \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/model_finetuned_results.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Comparing the fine-tuned \textit{PG-Video-LLaVA}~\cite{munasinghe2023PGVideoLLaVA} and \textit{Video-LLaMA}~\cite{damonlpsg2023videollama} regarding the \textit{BLEU}~\cite{bleu} (\textit{B}), \textit{ROUGE}~\cite{rouge} (\textit{R}) and \textit{BertScore}~\cite{bertscore} (\textit{BE}) metrics. The prompt "Create a question about the video content." is used for fine-tuning.}
\label{tab:finetuned_metrics}
\begin{tabular}{lrrr}
  \toprule
  \textbf{Model} & \textbf{B~\cite{bleu}} & \textbf{R~\cite{rouge}} & \textbf{BE~\cite{bertscore}}\\
  \midrule
  PG-Video-LLaVA & 4.19  & 0.19 & 0.87\\
  Video-LLaMA & 3.48 & 0.15 & 0.86\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/model_finetuned_results_new.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Comparing fine-tuned \textit{PG-Video-LLaVA} %~\cite{munasinghe2023PGVideoLLaVA} 
and \textit{Video-LLaMA} %~\cite{damonlpsg2023videollama} 
regarding \textit{BLEU} %~\cite{bleu} 
(\textit{B}), \textit{ROUGE} %~\cite{rouge} 
(\textit{R}) and \textit{BertScore} %~\cite{bertscore} 
(\textit{BE}). The prompt "Create a question about the video content." is used for fine-tuning.}
\label{tab:finetuned_metrics}
\begin{tabular}{lrrr}
  \toprule
  \textbf{Model} & \textbf{B~\cite{bleu}} & \textbf{R~\cite{rouge}} & \textbf{BE~\cite{bertscore}}\\
  \midrule
  PG-Video-LLaVA & 0.00 & 0.42 & 0.22\\
  Video-LLaMA & 0.00 & 0.25 & 0.21 \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/model_zeroshot_comparision_new.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Zero-shot performance regarding \textit{BLEU} %~\cite{bleu} 
(\textit{B}), \textit{ROUGE} %~\cite{rouge} 
(\textit{R}) and \textit{BertScore} %~\cite{bertscore} 
(\textit{BE}). 
%Mode describes the used prompt where 1 = "Create a question.", 2 = "Create a question about the video content." and 3 = "Create a question regarding the most important content of the video.". 
Mode describes the used prompt with numbering as defined in Section~\ref{subsec:zeroshot}.
\textit{Avg.} represents the average considering all results.}
\label{tab:zero_shot_metrics}
\begin{tabular}{lrrrrr}
  \toprule
  \textbf{Model} & \textbf{Mode} & \textbf{B~\cite{bleu}} & \textbf{R~\cite{rouge}} & \textbf{BE~\cite{bertscore}}\\
  \midrule
  Video-LLaVA & 1 & 0.00  & 0.47 & 0.33\\
  Video-LLaVA & 2 & 0.00 & 0.52 & 0.33\\
  Video-LLaVA & 3 & 0.00 & 0.48 & 0.30\\
  Video-LLaVA & Avg. & 0.00 & 0.49 & 0.32\\
  PG-Video-LLaVA & 1 & 0.00 & 0.27 & 0.14\\
  PG-Video-LLaVA & 2 & 0.00 & 0.27 & 0.12\\
  PG-Video-LLaVA & 3 & 0.00 & 0.21 & 0.07\\
  PG-Video-LLaVA & Avg. & 0.00 & 0.25 & 0.11\\  
  Video-LLaMA & 1 & 0.00 & 0.14 & -1.02\\
  Video-LLaMA & 2 & 0.00 & 0.13 & -1.06\\
  Video-LLaMA & 3 & 0.00 & 0.12 & -1.07\\
  Video-LLaMA & Avg. & 0.00 & 0.13 & -1.05\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/model_zeroshot_comparison.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Comparing the different non fine-tuned models regarding the \textit{BLEU}~\cite{bleu} (\textit{B}), \textit{ROUGE}~\cite{rouge} (\textit{R}) and \textit{BertScore}~\cite{bertscore} (\textit{BE}) metrics. Mode describes the used prompt where 1 = "Create a question.", 2 = "Create a question about the video content." and 3 = "Create a question regarding the most important content of the video.". The mode \textit{avg} represents the average of considering all results.}
\label{tab:zero_shot_metrics}
\begin{tabular}{lrrrrr}
  \toprule
  \textbf{Model} & \textbf{Mode} & \textbf{B~\cite{bleu}} & \textbf{R~\cite{rouge}} & \textbf{BE}\\
  \midrule
  Video-LLaVA & 1 & 3.73  & 0.17 & 0.88\\
  Video-LLaVA & 2 & 3.89 & 0.20 & 0.88\\
  Video-LLaVA & 3 & 3.89 & 0.19 & 0.88\\
  Video-LLaVA & Avg. & 3.84 & 0.19 & 0.88\\
  PG-Video-LLaVA & 1 & 3.49 & 0.18 & 0.87\\
  PG-Video-LLaVA & 2 & 3.59 & 0.17 & 0.88\\
  PG-Video-LLaVA & 3 & 3.75 & 0.18 & 0.88\\
  PG-Video-LLaVA & Avg & 3.61 & 0.17 & 0.88\\  
  Video-LLaMA & 1 & 0.08 & 0.00 & 0.04\\
  Video-LLaMA & 2 & 0.01 & 0.00 & 0.01\\
  Video-LLaMA & 3 & 0.00 & 0.00 & 0.00\\
  Video-LLaMA & Avg & 0.03 & 0.00 & 0.02\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/models_old.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Selected models and their characteristics for automatic question generation. \textit{All} for \textit{\#Frames} describes that frames are extracted at a regular interval. \textit{Audio} describes the use of the original audio signal present, whereas text represents the use of video information (speech transcript, audio signal).} 
%(e.g. speech transcript).}
\label{tab:vlm_models}
\begin{tabular}{lllll}
  \toprule
  \textbf{Model} & \textbf{\#Frames} & \textbf{Image} & \textbf{Audio} & \textbf{Text} \\
  \midrule
  Video-LLaVA~\cite{lin2023video} & 8 & \checkmark & \xmark & \xmark\\
  PG-Video-LLaVA~\cite{munasinghe2023PGVideoLLaVA} & All & \checkmark & \xmark & \checkmark\\
  Video-LLaMA~\cite{damonlpsg2023videollama} & All & \checkmark & \checkmark & \xmark\\
  Valley~\cite{luo2023valley} & All & \checkmark & \xmark & \xmark\\
  VideoChat~\cite{li2024videochat} & Keyframes & \xmark & \xmark & \checkmark\\
  VideoChatGPT~\cite{Maaz2023VideoChatGPT} & Keyframes & \xmark & \xmark & \xmark\\
  Mistral-7B-Instruct~\cite{mistral_7b} & 0 & \xmark & \xmark & \checkmark\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/prompt_finetuned.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Averaged fine-tuning evaluation of \textit{PG-Video-LLaVA}~\cite{munasinghe2023PGVideoLLaVA} and \textit{Video-LLaMA}~\cite{damonlpsg2023videollama}. \emph{Quest.} specifies the percentage of the results that are a question, while \textit{Statem.} is the percentage of statements produced. \textit{Empty} describes the percentage of empty output. The prompt "Create a question about the video content" is used for fine-tuning.}
\label{tab:finetune_questions}
\begin{tabular}{lrrr}
  \toprule
  \textbf{Model} & \textbf{Questions} & \textbf{Statements} & \textbf{Empty}\\
  \midrule
  %Video-LLaVA~\cite{lin2023video} & 7B & - & - & - \\
  %PG-Video-LLaVA~\cite{munasinghe2023PGVideoLLaVA} & 7B & 99.46\,\% & 0.54\,\% & 0.00\,\% \\
  PG-Video-LLaVA & 66.50\,\% & 28.70\,\% & 4.80\,\% \\
  %Video-LLaMA~\cite{damonlpsg2023videollama} & 7B & - & - & - \\
  Video-LLaMA & 98.06\,\% & 1.94\,\% & 0.00\,\% \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/qualitative_metrics_khan.tex <==
\begin{table*}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Examples of questions for Khan Academy sample (\url{https://youtu.be/BbZB-WBVFSk)} using the different settings of the fine-tuned \textit{PG-Video-LLaVA} and \textit{Video-LLaMA}. For each setting, the first question of each prompt is represented. Relevance (R), %specificness (S), 
coverage (C) and levels of understanding are considered (Level).}
\label{tab:quality_khan}
%\resizebox{\linewidth}{!}{
\begin{tabular}{llccl}
  \toprule
  \textbf{Model} & \textbf{Output} & \textbf{R} & %\textbf{S} & 
  \textbf{C} & \textbf{Level}\\
  \midrule
  PG-Video-LLaVA & What is the difference between an acid and a base? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  PG-Video-LLaVA & What is the difference between an amino acid and a peptide? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  PG-Video-LLaVA & What is the difference between an acid and a base? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  PG-Video-LLaVA (visual) & What is the difference between an acid and a base? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  PG-Video-LLaVA (visual) & What is the difference between an acid and a base? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  PG-Video-LLaVA (visual) & What is the difference between a base and a base pair? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  %PG-Video-LLaVA (audio) & - & \xmark & \xmark & \xmark & - \\  \midrule
  %PG-Video-LLaVA (audio) & - & \xmark & \xmark & \xmark & - \\  \midrule
  %PG-Video-LLaVA (audio) & - & \xmark & \xmark & \xmark & - \\  \midrule
  Video-LLaMA & \makecell[l]{So the hydroxide ion (OH) gets the charge of -2 and\\ the hydronium ion (H3O+) gets the charge of +1?} & \checkmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  Video-LLaMA & What is the pH of the blood after the H+ gets eliminated? & \checkmark & %\xmark & 
  \xmark & Applying \\  \midrule
  Video-LLaMA & \makecell[l]{If we were to isolate the cyano group, then would\\ that not cause the ion to become deprotonated?} & \xmark & %\xmark & 
  \xmark & Evaluating \\  \midrule
  Video-LLaMA (visual) & \makecell[l]{At 0:12, the concentration of ATP is the highest \\at the site of the reaction...I understand why,\\ but how does ATP get back to the cell?} & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  Video-LLaMA (visual) & If the pH inside a cell is 7, what is the pH of the extracellular fluids? & \xmark & %\xmark & 
  \xmark & Applying \\  \midrule
  Video-LLaMA (visual) & \makecell[l]{What would be the chemical equation for acetylcholine,\\ if it were in an acidic environment?} & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  Video-LLaMA (audio) & How does the doctor determine which type of arthritis you have? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  Video-LLaMA (audio) & Why did we use a barometer in the first place? & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  Video-LLaMA (audio) & Is a black hole a space object? & \xmark & %\xmark & 
  \xmark & Remembering \\
  \bottomrule
\end{tabular}
%}
\end{table*}

==> tables/qualitiative_metrics_teded.tex <==
\begin{table*}[ht]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{Examples of questions for TED-ED sample (\url{https://youtu.be/oz1Cz8ko8iY}) using the different settings of the fine-tuned \textit{PG-Video-LLaVA} and \textit{Video-LLaMA}. For each setting, the first question of each prompt is represented. Relevance (R), %specificness (S), 
coverage (C) and levels of understanding are considered (Level).}
\label{tab:quality_teded}
%\resizebox{\linewidth}{!}{
\begin{tabular}{llccl}
  \toprule
  \textbf{Model} & \textbf{Output} & \textbf{R} & %\textbf{S} & 
  \textbf{C} & \textbf{Level}\\
  \midrule
  PG-Video-LLaVA & What is the most frightening thing about the mystery of the vanishing bees? & \checkmark & %\checkmark & 
  \xmark & Remembering \\  \midrule
  PG-Video-LLaVA & What is the most frightening thing about the mystery of the vanishing bees? & \checkmark & %\checkmark & 
  \xmark & Remembering \\  \midrule
  PG-Video-LLaVA & What is the most likely cause of colony collapse disorder? & \checkmark & %\checkmark & 
  \xmark & Remembering \\  \midrule
  PG-Video-LLaVA (visual) & What is the difference between a hash function and a compression algorithm? & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  PG-Video-LLaVA (visual) & What is the difference between a hash function and a checksum? & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  PG-Video-LLaVA (visual) & What is the most important thing to remember about the mosquito? & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  %PG-Video-LLaVA (audio) & - & \xmark & %\xmark & 
  %\xmark & - \\  \midrule
  %PG-Video-LLaVA (audio) & - & \xmark & %\xmark & 
  %\xmark & - \\  \midrule
  %PG-Video-LLaVA (audio) & - & \xmark & %\xmark & 
  %\xmark & - \\  \midrule
  Video-LLaMA & What is the main idea of this video? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  Video-LLaMA & What is the main idea of this video? & \xmark & %\xmark & 
  \xmark & Understanding \\  \midrule
  Video-LLaMA & What are some examples of bioluminescent organisms? & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  Video-LLaMA (visual) & \makecell[l]{I was surprised to hear that the number of neurons in a bee's brain\\ was in excess of one million. I am curious about what types of information\\ is processed within the bee's brain. For example, does the bee process what\\ is edible/inedible, and what are some examples of memory the bee uses?} & \checkmark & %\checkmark & 
  \checkmark & Remembering \\  \midrule
  Video-LLaMA (visual) & Is there more than 1 species of varroa mite? & \checkmark & %\checkmark & 
  \checkmark & Remembering \\  \midrule
  Video-LLaMA (visual) & Why does the brain have more cells in it than there are stars in the universe? & \xmark & %\xmark & 
  \checkmark & Understanding \\  \midrule
  Video-LLaMA (audio) & How many elements can a compound have? & \xmark & %\xmark & 
  \xmark & Remembering \\  \midrule
  Video-LLaMA (audio) & \makecell[l]{If you have an object with a velocity of 20 meters per second in the\\ negative direction, how fast is it moving from an observer who is moving in \\ the positive direction at a velocity of 10 meters per second?} & \xmark & %\xmark & 
  \xmark & Applying \\  \midrule
  Video-LLaMA (audio) & What is the difference between a 'magnification' and 'microscopic' object? & \xmark & %\xmark & 
  \xmark & Remembering \\ 
  \bottomrule
\end{tabular}
%}
\end{table*}

==> tables/teded_stats.tex <==
\begin{table}[htbp]
%\setlength{\tabcolsep}{2.1pt}
\centering
%\fontsize{8}{10}\selectfont
%\def\arraystretch{0.9}
\caption{The distribution of multiple-choice questions and open-ended questions from TED-Ed inside the different data splits (numbers and percentage ratio of multiple-choice questions (MCQs) to open-ended  questions (OEQs)).}
%\resizebox{\columnwidth}{!}{
\label{tab:teded_stats}
\begin{tabular}{lrrr}
  \hline
  \textbf{Question-Type} & \textbf{MCQs} & \textbf{OEQs} & \textbf{Ratio [\%]}\\
  \hline
  \textbf{\#Train} & 3,047 & 2,554 & 54.40\\
  \textbf{\#Val} & 404 & 322 & 55.56\\
  \textbf{\#Test} & 366 & 314 & 53.82\\
  \hline
\end{tabular}
%}
\end{table}
